A Generic Branch-and-Bound Algorithm for $\ell_0$-Penalized Problems with Supplementary Material

We present a generic Branch-and-Bound procedure designed to solve L0-penalized optimization problems. Existing approaches primarily focus on quadratic losses and construct relaxations using "Big-M" constraints and/or L2-norm penalties. In contrast, our method accommodates a broader class of loss functions and allows greater flexibility in relaxation design through a general penalty term, encompassing existing techniques as special cases. We establish theoretical results ensuring that all key quantities required for the Branch-and-Bound implementation admit closed-form expressions under the general blanket assumptions considered in our work. Leveraging this framework, we introduce El0ps, an open-source Python solver with a plug-and-play workflow that enables user-defined losses and penalties in L0-penalized problems. Through extensive numerical experiments, we demonstrate that El0ps achieves state-of-the-art performance on classical instances and extends computational feasibility to previously intractable ones.

==> img/regpath/regpath-loss.tex <==
\pgfplotscreateplotcyclelist{cycle_list_regpath_loss}{
    black, thick, mark=*, mark options={scale=0.5}\\     
}

\begin{tikzpicture}
    \begin{groupplot}[
        group style     = {
            group size      = 3 by 2,
            vertical sep    = 55pt,
            horizontal sep  = 47pt,
        },
        height          = 4.0cm,
        width           = 4.3cm,
        ytick pos       = left,
        xtick pos       = bottom,
        grid            = major,
        xlabel          = $\reg/\regmax$,
        xmode           = log,
        x dir           = reverse,
        xmin            = 0.006,
        ylabel          = Loss value,
        ymax            = 1.1,
        ymin            = -0.1,
        ylabel style    = {at={(-0.3,0.5)}},
        cycle list name = cycle_list_regpath_loss,
    ]

        % -------------
        % riboflavin
        % -------------


        \nextgroupplot[title = \textsc{Riboflavin}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=riboflavin-datafit=Leastsquares-penalty=BigmL2norm.csv};

        % -------------
        % colon-cancer
        % -------------

        \nextgroupplot[title = \textsc{Colon cancer}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=colon-cancer-datafit=Logistic-penalty=BigmL2norm.csv};

        % -------------
        % breast-cancer
        % -------------

        \nextgroupplot[title = \textsc{Breast cancer}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=breast-cancer-datafit=Squaredhinge-penalty=BigmL2norm.csv};

        % -------------
        % bctcga
        % -------------

        \nextgroupplot[title = \textsc{Bctcga}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=bctcga-datafit=Leastsquares-penalty=BigmL2norm.csv};

        % -------------
        % leukemia
        % -------------

        \nextgroupplot[title = \textsc{Leukemia}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=leukemia-datafit=Logistic-penalty=BigmL2norm.csv};

        % -------------
        % arcene
        % -------------

        \nextgroupplot[title = \textsc{Arcene}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=arcene-datafit=Squaredhinge-penalty=BigmL2norm.csv};

    \end{groupplot}
\end{tikzpicture}

\begin{center}
    \rule{0.75\linewidth}{0.5pt}
\end{center}
\vspace{0.25cm}

\begin{tikzpicture}
    \begin{groupplot}[
        group style     = {
            group size      = 3 by 2,
            vertical sep    = 55pt,
            horizontal sep  = 47pt,
        },
        height          = 4.0cm,
        width           = 4.3cm,
        ytick pos       = left,
        xtick pos       = bottom,
        grid            = major,
        xlabel          = $\reg/\regmax$,
        xmode           = log,
        x dir           = reverse,
        xmin            = 0.006,
        ylabel          = Loss value,
        ymax            = 1.1,
        ymin            = -0.1,
        ylabel style    = {at={(-0.3,0.5)}},
        cycle list name = cycle_list_regpath_loss,
    ]

        % -------------
        % riboflavin
        % -------------


        \nextgroupplot[title = \textsc{Riboflavin}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=riboflavin-datafit=Leastsquares-penalty=BigmL1norm.csv};

        % -------------
        % colon-cancer
        % -------------

        \nextgroupplot[title = \textsc{Colon cancer}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=colon-cancer-datafit=Logistic-penalty=BigmL1norm.csv};

        % -------------
        % breast-cancer
        % -------------

        \nextgroupplot[title = \textsc{Breast cancer}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=breast-cancer-datafit=Squaredhinge-penalty=BigmL1norm.csv};

        % -------------
        % bctcga
        % -------------

        \nextgroupplot[title = \textsc{Bctcga}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=bctcga-datafit=Leastsquares-penalty=BigmL1norm.csv};

        % -------------
        % leukemia
        % -------------

        \nextgroupplot[title = \textsc{Leukemia}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=leukemia-datafit=Logistic-penalty=BigmL1norm.csv};

        % -------------
        % arcene
        % -------------

        \nextgroupplot[title = \textsc{Arcene}]
        \addplot table[
            x       = lgrid, 
            y       = datafit_value,
            col sep = comma,
        ] {img/regpath/regpath-dataset=arcene-datafit=Squaredhinge-penalty=BigmL1norm.csv};

    \end{groupplot}
\end{tikzpicture}

==> img/regpath/regpath-nnz.tex <==
\pgfplotscreateplotcyclelist{cycle_list_regpath_nnz}{
    black, thick, mark=*, mark options={scale=0.5}\\     
}

\begin{tikzpicture}
    \begin{groupplot}[
        group style     = {
            group size      = 3 by 2,
            vertical sep    = 55pt,
            horizontal sep  = 47pt,
        },
        height          = 4.0cm,
        width           = 4.3cm,
        ytick pos       = left,
        xtick pos       = bottom,
        grid            = major,
        xlabel          = $\reg/\regmax$,
        xmode           = log,
        x dir           = reverse,
        xmin            = 0.006,
        ylabel          = Non-zeros,
        ylabel style    = {at={(-0.3,0.5)}},
        cycle list name = cycle_list_regpath_nnz,
    ]

        % -------------
        % riboflavin
        % -------------


        \nextgroupplot[title = \textsc{Riboflavin}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=riboflavin-datafit=Leastsquares-penalty=BigmL2norm.csv};

        % -------------
        % colon-cancer
        % -------------

        \nextgroupplot[title = \textsc{Colon cancer}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=colon-cancer-datafit=Logistic-penalty=BigmL2norm.csv};

        % -------------
        % breast-cancer
        % -------------

        \nextgroupplot[title = \textsc{Breast cancer}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=breast-cancer-datafit=Squaredhinge-penalty=BigmL2norm.csv};

        % -------------
        % bctcga
        % -------------

        \nextgroupplot[title = \textsc{Bctcga}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=bctcga-datafit=Leastsquares-penalty=BigmL2norm.csv};

        % -------------
        % leukemia
        % -------------

        \nextgroupplot[title = \textsc{Leukemia}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=leukemia-datafit=Logistic-penalty=BigmL2norm.csv};

        % -------------
        % arcene
        % -------------

        \nextgroupplot[title = \textsc{Arcene}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=arcene-datafit=Squaredhinge-penalty=BigmL2norm.csv};

    \end{groupplot}
\end{tikzpicture}

\begin{center}
    \rule{0.75\linewidth}{0.5pt}
\end{center}
\vspace{0.25cm}

\begin{tikzpicture}
    \begin{groupplot}[
        group style     = {
            group size      = 3 by 2,
            vertical sep    = 55pt,
            horizontal sep  = 47pt,
        },
        height          = 4.0cm,
        width           = 4.3cm,
        ytick pos       = left,
        xtick pos       = bottom,
        grid            = major,
        xlabel          = $\reg/\regmax$,
        xmode           = log,
        x dir           = reverse,
        xmin            = 0.006,
        ylabel          = Non-zeros,
        ylabel style    = {at={(-0.3,0.5)}},
        cycle list name = cycle_list_regpath_nnz,
    ]

        % -------------
        % riboflavin
        % -------------


        \nextgroupplot[title = \textsc{Riboflavin}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=riboflavin-datafit=Leastsquares-penalty=BigmL1norm.csv};

        % -------------
        % colon-cancer
        % -------------

        \nextgroupplot[title = \textsc{Colon cancer}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=colon-cancer-datafit=Logistic-penalty=BigmL1norm.csv};

        % -------------
        % breast-cancer
        % -------------

        \nextgroupplot[title = \textsc{Breast cancer}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=breast-cancer-datafit=Squaredhinge-penalty=BigmL1norm.csv};

        % -------------
        % bctcga
        % -------------

        \nextgroupplot[title = \textsc{Bctcga}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=bctcga-datafit=Leastsquares-penalty=BigmL1norm.csv};

        % -------------
        % leukemia
        % -------------

        \nextgroupplot[title = \textsc{Leukemia}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=leukemia-datafit=Logistic-penalty=BigmL1norm.csv};

        % -------------
        % arcene
        % -------------

        \nextgroupplot[title = \textsc{Arcene}]
        \addplot table[
            x       = lgrid, 
            y       = n_nnz,
            col sep = comma,
        ] {img/regpath/regpath-dataset=arcene-datafit=Squaredhinge-penalty=BigmL1norm.csv};

    \end{groupplot}
\end{tikzpicture}

